On the interpretation of IceCube cascade events in terms of the Glashow resonance

The IceCube experiment (IC) has recently observed 2 cascade events with energies between 1 and 10 PeV. This energy combined with the fact that no muon-track events are observed may be interpreted as a cosmogenic $\bar \nu_e$ interacting in IC via the Glashow resonance (GR) $\bar \nu_e e \to W^-\to$ (hadrons or $\bar \nu_e e$). We point out a unique, background-free signature of the GR, a single isolated muon unaccompanied by any shower activity from the interaction $\bar \nu_e e \to W^-\to \bar \nu_\mu \mu^-$, and propose it as a test of this interpretation. We calculate the event numbers and find that a single such event is expected over about a three-year period in IC. We also show that, if event rates remain at their current levels then, even with the GR, standard cosmogenic fluxes cannot easily explain the observations. Moreover, if muon-tracks remain conspicuous by their absence, then new physics needs to be invoked. As example scenarios in conformity with the observations, we calculate event rates for neutrino decay and Lorentz-invariance violation.

==> PaxHeaders.9974/GR_neu.tex <==
30 atime=1347392261.650325622
30 ctime=1347392247.002167746

